Brownian Motions on Metric Graphs with Non-Local Boundary Conditions II: Construction

A pathwise construction of discontinuous Brownian motions on metric graphs is given for every possible set of non-local Feller-Wentzell boundary conditions. This construction is achieved by locally decomposing the metric graphs into star graphs, establishing local solutions on these partial graphs, pasting the solutions together, introducing non-local jumps, and verifying the generator of the resulting process.

==> 0_commands_wt.tex <==
%% for double widetilde, as seen at
%%  http://tex.stackexchange.com/questions/3682/how-do-i-lower-the-widetilde-accent-i-e-move-it-closer-to-the-variable
 
\makeatletter
\newcommand*\wt[1]{\mathpalette\wthelper{#1}}
\newcommand*\wthelper[2]{%
        \hbox{\dimen@\accentfontxheight#1%
                \accentfontxheight#11.3\dimen@
                $\m@th#1\widetilde{#2}$%
                \accentfontxheight#1\dimen@
        }%
}


\newcommand*\doubletilde[1]{\mathpalette\dthelper{#1}}
\newcommand*\dthelper[2]{%
        \hbox{\dimen@\accentfontxheight#1%
                \accentfontxheight#11.3\dimen@
                \sbox\z@{$\m@th#1\! \tilde{#2}$}%
                \ht\z@=.9\ht\z@
                $\tilde{\box\z@}$%
                \accentfontxheight#1\dimen@
        }%
}


\newcommand*\accentfontxheight[1]{%
        \fontdimen5\ifx#1\displaystyle
                \textfont
        \else\ifx#1\textstyle
                \textfont
        \else\ifx#1\scriptstyle
                \scriptfont
        \else
                \scriptscriptfont
        \fi\fi\fi3
}
\makeatother

